Do Encoder Representations of Generative Dialogue Models Encode Sufficient Information about the Task ?

Predicting the next utterance in dialogue is contingent on encoding of users' input text to generate appropriate and relevant response in data-driven approaches. Although the semantic and syntactic quality of the language generated is evaluated, more often than not, the encoded representation of input is not evaluated. As the representation of the encoder is essential for predicting the appropriate response, evaluation of encoder representation is a challenging yet important problem. In this work, we showcase evaluating the text generated through human or automatic metrics is not sufficient to appropriately evaluate soundness of the language understanding of dialogue models and, to that end, propose a set of probe tasks to evaluate encoder representation of different language encoders commonly used in dialogue models. From experiments, we observe that some of the probe tasks are easier and some are harder for even sophisticated model architectures to learn. And, through experiments we observe that RNN based architectures have lower performance on automatic metrics on text generation than transformer model but perform better than the transformer model on the probe tasks indicating that RNNs might preserve task information better than the Transformers.

==> dumps/arXiv_non_linear_tables.tex <==
 \begin{table}[h!]
\tiny
\centering
      \begin{tabular}{c|a|b|a}
         \hline
         \multicolumn{4}{c}{PersonaChat Dataset}\\
         \hline
         {\bf Model} & {\bf UtteranceLoc} & {\bf WordCont} & {\bf PersonalInfo} \\
         \hline
         \rowcolor{LightBlue}\multicolumn{4}{c}{Bi-LSTM Seq2Seq + Attention} \\
         \hline
         Untrained & 38.61 $\pm$ 0.00 &39.76 $\pm$ 0.03 &0.61 $\pm$ 0.00\\
         LastEpoch & 59.05 $\pm$ 0.08 &35.82 $\pm$ 0.05 &1.29 $\pm$ 0.00  \\
         BestBLEU & 57.50 $\pm$ 0.01 &36.06 $\pm$ 0.05 &1.43 $\pm$ 0.00   \\
        \hline
         \rowcolor{LightBlue}\multicolumn{4}{c}{HRED - LSTM} \\
         \hline
         Untrained & 38.20 $\pm$ 0.03 &50.91 $\pm$ 0.08 &0.00 $\pm$ 0.00\\
         LastEpoch & 11.74 $\pm$ 4.13 &51.73 $\pm$ 0.02 &0.00 $\pm$ 0.00   \\
         BestBLEU & 12.41 $\pm$ 4.62 &51.97 $\pm$ 0.01 &0.00 $\pm$ 0.00  \\
         \hline
         \rowcolor{LightBlue}\multicolumn{4}{c}{LSTM Seq2Seq + Attention} \\
         \hline
         Untrained & 38.47 $\pm$ 1.21 &43.41 $\pm$ 0.02 &0.67 $\pm$ 0.00 \\
         LastEpoch & 52.45 $\pm$ 0.03 &34.16 $\pm$ 0.09 &1.15 $\pm$ 0.00 \\
         BestBLEU & 49.73 $\pm$ 0.23 &28.05 $\pm$ 1.78 &0.88 $\pm$ 0.01   \\
         \hline
         \rowcolor{LightBlue}\multicolumn{4}{c}{LSTM Seq2Seq} \\
         \hline
         Untrained & 44.18 $\pm$ 0.03 &43.08 $\pm$ 0.01 &0.74 $\pm$ 0.00\\
         LastEpoch & 51.23 $\pm$ 0.07 &36.12 $\pm$ 0.01 &1.07 $\pm$ 0.00  \\
         BestBLEU & 54.54 $\pm$ 0.02 &34.75 $\pm$ 0.03 &1.33 $\pm$ 0.00   \\
         \hline
         \rowcolor{LightBlue}\multicolumn{4}{c}{Transformer Architecture} \\
         \hline
         Untrained & 64.04 $\pm$ 0.01 &31.19 $\pm$ 0.77 &1.17 $\pm$ 0.00 \\
         LastEpoch & 51.74 $\pm$ 0.00 &47.99 $\pm$ 0.58 &0.00 $\pm$ 0.00 \\
         BestBLEU & 51.77 $\pm$ 0.00 &39.22 $\pm$ 4.09 &0.01 $\pm$ 0.00  \\
         \hline
    \end{tabular}
    \caption{Comparison of models on probe tasks in PersonaChat dialogue data set with a multi-layer perceptron on the different encoder representation. The performance is measured with \emph{F1} on the probetasks. The trend in the performance of the models is similar to with Logistic Regression, where the performance on WordCont task decreases with increase in training epochs, and the PersonalInfo task is still difficult for the models.}
    \label{tab:non-linear-persona-probe-tasks-metric}
\end{table}
  \begin{table*}[h!]
        \tiny
        \centering
        \begin{tabular}{c|a|b|a|b|a|b|a|b}
         \hline
         \multicolumn{9}{c}{MultiWoZ Dataset}\\
         \hline
         {\bf Model} & {\bf UtteranceLoc} & {\bf RecentTopic} & {\bf RecentSlots} & {\bf RecentValues} & {\bf RepeatInfo} & {\bf NumRepeatInfo}& {\bf NumRecentInfo} & {\bf AllSlots} \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{LSTM Seq2Seq + Attention} \\
         \hline
         Untrained &46.47 $\pm$ 0.49 &35.34 $\pm$ 0.00 &39.04 $\pm$ 0.01 &30.82 $\pm$ 0.00 &64.23 $\pm$ 0.02 &68.95 $\pm$ 0.01 &41.40 $\pm$ 0.03 &30.21 $\pm$ 0.00  \\
         LastEpoch &56.50 $\pm$ 0.06 &87.11 $\pm$ 0.01 &65.61 $\pm$ 0.00 &42.19 $\pm$ 0.00 &64.91 $\pm$ 0.00 &70.03 $\pm$ 0.01 &61.74 $\pm$ 0.06 &51.51 $\pm$ 0.01 \\
         BestBLEU &58.03 $\pm$ 0.05 &88.95 $\pm$ 0.04 &66.53 $\pm$ 0.00 &41.09 $\pm$ 0.01 &64.47 $\pm$ 0.00 &66.89 $\pm$ 0.02 &63.37 $\pm$ 0.02 &52.02 $\pm$ 0.05 \\
        \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{HRED - LSTM} \\
         \hline
         Untrained & 45.28 $\pm$ 1.56 &32.90 $\pm$ 0.02 &41.20 $\pm$ 0.03 &31.69 $\pm$ 0.02 &70.98 $\pm$ 0.01 &74.85 $\pm$ 0.01 &40.65 $\pm$ 0.03 &19.79 $\pm$ 0.03 \\
         LastEpoch & 37.96 $\pm$ 10.86 &54.21 $\pm$ 22.63 &36.27 $\pm$ 10.10 &21.27 $\pm$ 3.41 &69.42 $\pm$ 0.06 &74.02 $\pm$ 0.02 &39.45 $\pm$ 11.67 &32.77 $\pm$ 8.39 \\
         BestBLEU & 38.71 $\pm$ 11.27 &50.10 $\pm$ 20.50 &34.27 $\pm$ 9.34 &20.45 $\pm$ 3.14 &70.98 $\pm$ 0.07 &74.53 $\pm$ 0.09 &39.29 $\pm$ 11.58 &30.26 $\pm$ 7.87 \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{LSTM Seq2Seq } \\
         \hline
         Untrained &46.56 $\pm$ 0.31 &35.85 $\pm$ 0.00 &39.68 $\pm$ 0.00 &32.03 $\pm$ 0.01 &64.82 $\pm$ 0.03 &69.18 $\pm$ 0.04 &42.98 $\pm$ 0.01 &29.49 $\pm$ 0.00 \\
         LastEpoch &54.95 $\pm$ 0.06 &87.64 $\pm$ 0.01 &66.04 $\pm$ 0.01 &41.94 $\pm$ 0.01 &66.11 $\pm$ 0.00 &69.84 $\pm$ 0.01 &61.03 $\pm$ 0.04 &51.63 $\pm$ 0.01 \\
         BestBLEU&56.27 $\pm$ 0.03 &88.57 $\pm$ 0.02 &66.88 $\pm$ 0.00 &41.55 $\pm$ 0.04 &65.89 $\pm$ 0.00 &70.20 $\pm$ 0.01 &62.62 $\pm$ 0.00 &52.61 $\pm$ 0.03 \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{Bi-LSTM Seq2Seq + Attention} \\
         \hline
         Untrained &44.26 $\pm$ 0.02 &50.65 $\pm$ 0.07 &35.26 $\pm$ 0.01 &27.27 $\pm$ 0.01 &64.58 $\pm$ 0.02 &70.55 $\pm$ 0.00 &39.93 $\pm$ 0.00 &36.67 $\pm$ 0.01 \\
         LastEpoch &57.21 $\pm$ 0.04 &86.66 $\pm$ 0.01 &63.29 $\pm$ 0.01 &38.17 $\pm$ 0.02 &66.55 $\pm$ 0.00 &70.76 $\pm$ 0.00 &60.23 $\pm$ 0.07 &53.36 $\pm$ 0.00 \\
         BestBLEU &57.47 $\pm$ 0.07 &88.98 $\pm$ 0.01 &64.54 $\pm$ 0.01 &39.56 $\pm$ 0.01 &68.48 $\pm$ 0.00 &72.19 $\pm$ 0.00 &62.34 $\pm$ 0.03 &56.02 $\pm$ 0.02 \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{Transformer Architecture} \\
         \hline
         Untrained &51.24 $\pm$ 0.04 &80.25 $\pm$ 0.03 &45.58 $\pm$ 0.01 &30.61 $\pm$ 0.01 &70.36 $\pm$ 0.02 &73.25 $\pm$ 0.00 &47.47 $\pm$ 0.03 &62.94 $\pm$ 0.01 \\
         LastEpoch & 33.73 $\pm$ 0.48 &32.14 $\pm$ 1.87 &26.17 $\pm$ 1.87 &22.11 $\pm$ 1.65 &70.75 $\pm$ 0.04 &74.63 $\pm$ 0.03 &33.64 $\pm$ 3.26 &21.25 $\pm$ 0.57 \\
         BestBLEU &31.96 $\pm$ 0.47 &31.69 $\pm$ 5.29 &29.64 $\pm$ 0.34 &25.34 $\pm$ 0.21 &72.16 $\pm$ 0.00 &75.90 $\pm$ 0.00 &37.77 $\pm$ 0.37 &22.75 $\pm$ 1.44 \\
         \hline
    \end{tabular}
    \caption{The performance of multi-layer perceptron over the encoder representation of different generative dialogue models on probe tasks in MultiWoZ dialogue data set . The performance is measured with \emph{F1}. The results, similar to the probe tasks with Logistic Regression, show that SEQ2SEQ models perform significantly better than Transformer model on the probe tasks, despite the models falling behind in BLEU score.}
    \label{tab:non-linear-multiwoz-probe-tasks-1}
\end{table*}

\begin{table*}[h!]
\tiny
\centering
    \begin{tabular}{c|a|b|a|b|a|b|a|b}
         \hline
         \multicolumn{9}{c}{MultiWoZ Dataset}\\
         \hline
         {\bf Model} & {\bf AllValues} & {\bf NumAllInfo} & {\bf AllTopics}&{\bf NumAllTopics} & {\bf IsMultiTask} & {\bf EntitySlots} & {\bf EntityValues} & {\bf ActionSelect} \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{LSTM Seq2Seq + Attention} \\
         \hline
         Untrained &12.63 $\pm$ 0.01 &6.97 $\pm$ 0.01 &45.10 $\pm$ 0.00 &70.27 $\pm$ 0.02 &80.06 $\pm$ 0.01 &28.04 $\pm$ 0.00 &19.63 $\pm$ 0.00 &28.66 $\pm$ 0.00 \\
         LastEpoch & 19.33 $\pm$ 0.00 &29.28 $\pm$ 0.03 &73.35 $\pm$ 0.00 &76.25 $\pm$ 0.03 &81.54 $\pm$ 0.04 &43.48 $\pm$ 0.02 &28.42 $\pm$ 0.00 &56.21 $\pm$ 0.01 \\
         BestBLEU  &18.65 $\pm$ 0.00 &29.16 $\pm$ 0.03 &74.34 $\pm$ 0.02 &76.93 $\pm$ 0.05 &82.12 $\pm$ 0.00 &42.55 $\pm$ 0.01 &29.09 $\pm$ 0.00 &56.88 $\pm$ 0.00 \\
        \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{HRED - LSTM} \\
         \hline
         Untrained & 5.28 $\pm$ 0.00 &0.00 $\pm$ 0.00 &37.51 $\pm$ 0.04 &77.57 $\pm$ 0.00 &84.24 $\pm$ 0.00 &24.86 $\pm$ 0.07 &19.01 $\pm$ 0.04 &27.26 $\pm$ 0.01 \\
         LastEpoch &8.73 $\pm$ 0.69 &19.05 $\pm$ 2.80 &48.66 $\pm$ 18.04 &69.23 $\pm$ 3.68 &73.51 $\pm$ 4.69 &27.07 $\pm$ 5.64 &20.22 $\pm$ 3.07 &38.76 $\pm$ 11.28 \\
         BestBLEU  &8.44 $\pm$ 0.78 &18.03 $\pm$ 2.63 &46.61 $\pm$ 16.88 &68.56 $\pm$ 3.48 &73.19 $\pm$ 4.58 &24.80 $\pm$ 4.94 &20.06 $\pm$ 3.02 &34.40 $\pm$ 9.31 \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{LSTM Seq2Seq } \\
         \hline
         Untrained &13.29 $\pm$ 0.00 &6.29 $\pm$ 0.02 &43.04 $\pm$ 0.01 &73.33 $\pm$ 0.01 &80.38 $\pm$ 0.05 &27.28 $\pm$ 0.01 &20.34 $\pm$ 0.00 &29.00 $\pm$ 0.01 \\
         LastEpoch  &19.48 $\pm$ 0.00 &28.80 $\pm$ 0.01 &72.84 $\pm$ 0.01 &75.74 $\pm$ 0.01 &81.22 $\pm$ 0.00 &44.00 $\pm$ 0.01 &30.72 $\pm$ 0.01 &56.67 $\pm$ 0.01 \\
         BestBLEU  &18.78 $\pm$ 0.00 &29.67 $\pm$ 0.02 &74.28 $\pm$ 0.03 &77.08 $\pm$ 0.03 &81.89 $\pm$ 0.00 &44.21 $\pm$ 0.00 &28.88 $\pm$ 0.03 &57.16 $\pm$ 0.02 \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{Bi-LSTM Seq2Seq + Attention} \\
         \hline
         Untrained &14.94 $\pm$ 0.00 &10.88 $\pm$ 0.08 &56.79 $\pm$ 0.00 &71.36 $\pm$ 0.01 &79.49 $\pm$ 0.01 &24.21 $\pm$ 0.00 &19.04 $\pm$ 0.01 &26.07 $\pm$ 0.02 \\
         LastEpoch &20.00 $\pm$ 0.00 &28.54 $\pm$ 0.01 &74.83 $\pm$ 0.01 &78.37 $\pm$ 0.01 &83.97 $\pm$ 0.00 &42.08 $\pm$ 0.00 &29.55 $\pm$ 0.02 &55.43 $\pm$ 0.01 \\
         BestBLEU & 20.03 $\pm$ 0.01 &29.56 $\pm$ 0.04 &77.37 $\pm$ 0.00 &79.06 $\pm$ 0.01 &84.21 $\pm$ 0.01 &41.62 $\pm$ 0.03 &28.21 $\pm$ 0.00 &56.53 $\pm$ 0.00 \\
         \hline
         \rowcolor{LightBlue}\multicolumn{9}{c}{Transformer Architecture} \\
         \hline
         Untrained  & 39.62 $\pm$ 0.00 &27.26 $\pm$ 0.03 &81.16 $\pm$ 0.00 &77.63 $\pm$ 0.00 &82.79 $\pm$ 0.00 &30.29 $\pm$ 0.02 &19.72 $\pm$ 0.11 &38.48 $\pm$ 0.19 \\
         LastEpoch  &5.11 $\pm$ 0.12 &11.48 $\pm$ 0.50 &47.65 $\pm$ 1.28 &71.93 $\pm$ 0.00 &82.00 $\pm$ 0.01 &13.48 $\pm$ 0.40 &13.35 $\pm$ 0.04 &6.76 $\pm$ 0.09\\
         BestBLEU  & 5.56 $\pm$ 0.14 &7.30 $\pm$ 0.23 &50.38 $\pm$ 1.14 &73.49 $\pm$ 0.04 &81.71 $\pm$ 0.01 &23.28 $\pm$ 0.14 &12.21 $\pm$ 0.33 &7.79 $\pm$ 0.22 \\
         \hline
    \end{tabular}
    \caption{The performance of different generative dialogue models on probe tasks in MultiWoZ dialogue data set. The performance is measured with $F-1$. The results show that SEQ2SEQ models show signs of learning on the probe tasks indirectly by learning to generate next utterance. Whereas the Transformer model's performance decreased from initial to last epoch in majority of the tasks.}
    \label{tab:non-linear-multiwoz-probe-tasks}
\end{table*}
